SILO Language Models: Isolating Legal Risk In a Nonparametric Datastore

The legality of training language models (LMs) on copyrighted or otherwise restricted data is under intense debate. However, as we show, model performance significantly degrades if trained only on low-risk text (e.g., out-of-copyright books or government documents), due to its limited size and domain coverage. We present SILO, a new language model that manages this risk-performance tradeoff during inference. SILO is built by (1) training a parametric LM on Open License Corpus (OLC), a new corpus we curate with 228B tokens of public domain and permissively licensed text and (2) augmenting it with a more general and easily modifiable nonparametric datastore (e.g., containing copyrighted books or news) that is only queried during inference. The datastore allows use of high-risk data without training on it, supports sentence-level data attribution, and enables data producers to opt out from the model by removing content from the store. These capabilities can foster compliance with data-use regulations such as the fair use doctrine in the United States and the GDPR in the European Union. Our experiments show that the parametric LM struggles on domains not covered by OLC. However, access to the datastore greatly improves out of domain performance, closing 90% of the performance gap with an LM trained on the Pile, a more diverse corpus with mostly high-risk text. We also analyze which nonparametric approach works best, where the remaining errors lie, and how performance scales with datastore size. Our results suggest that it is possible to build high quality language models while mitigating their legal risk.

==> sections/07-related.tex <==
\tightparagraph{Nonparametric language models.}
LMs that use a nonparametric datastore at test time---often called retrieval-based LMs---are adept at improving parameter efficiency, long-tail performance, and domain adaptation~\citep{guu2020retrieval,khandelwal2020generalization,he-etal-2021-efficient,borgeaud2022improving,min2022nonparametric,shi2023replug,ram2023context,huang2023k}. There are two broad approaches that we consider: retrieval-in-context models (\riclm) which concatenate the test input with text snippets retrieved from the datastore~\citep{shi2023replug,ram2023context}, and \knnlm\ models that use a non-parametric prediction function~\citep{{khandelwal2020generalization}}.


Our key contribution is
to leverage the properties of nonparametric LMs for better aligning with copyright laws. This is achieved by fitting parameters exclusively on permissively-licensed data, while simultaneously storing non-permissive data in the datastore.
Moreover, our experiments include a series of novel analyses, including comparison between \riclm\ and \knnlm\ with respect to the datastore size, both with and without distribution shift, and the effect of distribution shift on a parametric LM (which produces a parametric distribution) and on the encoder (which produces a nonparametric distribution).

\tightparagraph{Modular language models.} Our work is closely related to recent studies on modular LMs, which have specialized parameters (or \emph{experts}) trained on different domains \citep{gururangan-etal-2022-demix, li2022branch, gururangan2023scaling}, languages \citep{pfeiffer2020madx, pfeiffer2022lifting}, or tasks \citep{chen2022modsquad, jang2023exploring}. Our work extends modular LMs to include nonparametric datastores, and focuses on "specializing" different parts of the model to low- and high-risk subsets of the training data. Legal risks may also be mitigated with a collection of parametric expert models that are specialized to low- and high-risk data. Future work may explore this possibility, as well as the usefulness of combining a non-parametric datastore with parametric experts. Our parametric LMs (trained only on low-risk data) may also be a useful initialization for large collection of experts, to provide better guarantees on their provenance.
